Scalar mass conservation in turbulent mixture fraction based combustion models through consistent local flow parameters

Mixture fraction-based models are widely employed for predicting turbulent non-premixed combustion processes due to their cost-effectiveness and well-established subfilter closure. In these models, the transport of reactive scalars in physical space is decomposed into two components: scalar transport relative to mixture fraction and transport of mixture fraction in physical space. Conventional flamelet models do not consider that these two processes have to be formulated consistently, which can lead to scalar mass conservation errors. In the context of multiphase flows, scalar transport in mixture fraction space is governed by three conditional flow-dependent parameters: the conditional scalar dissipation rate, the conditional scalar diffusion rate, and the conditional spray source term. The evolution of mixture fraction in physical space is typically modeled using the presumed Filtered Density Function (FDF) approach. This paper introduces a novel formulation for the conditional flow parameters that aligns with the presumed FDF approach, thereby ensuring scalar mass conservation. The proposed model is applied to a Large-Eddy Simulation (LES) of the inert ECN Spray A case, with a comparison against a conventional flow parameter model that employs an inverse error function shape for the scalar dissipation rate. The results indicate that the conventional model produces similar conditional dissipation rates to the new model in regions where combustion takes place. However, significant discrepancies are observed in the conditional diffusion rate, highlighting the susceptibility of the conventional model to scalar mass conservation errors for non-unity Lewis number scalars.

==> detailed_model.tex <==
% !TEX root = CNF_davidovic.tex
\onecolumn
\setcounter{page}{1} 
\setcounter{section}{0} 
\setcounter{equation}{0} 
\noindent\textbf{Detailed model derivation} \newline\newline
The derivation of the turbulent non-premixed flamelet equations and the consistent flow parameters is described in the following. In the first section, the governing equations and the LES concept will be presented. The second section describes the concept of the fine-grained FDF, including some valuable properties for manipulating the equation. The third section presents the flamelet assumption and the flamelet model derivation. The section closes with a flow parameter formulation that is consistent with the presumed FDF evolution.

\section{Governing Equations}\noindent
The turbulent flamelet equation for a reactive scalar can be derived from the balance equations for density $\rho$, mixture fraction $Z$, and the scalar $\phi$. Assuming constant Lewis numbers and employing the binary flux approximation for diffusion, the governing equations can be written as
\begin{align}
\dt{\rho } + \dxi{\rho u_i } &= \dot{S}_\rho, \label{sm_eq:Continuity} \\
\dt{\rho Z} + \dxi{\rho u_i Z} &= \dxi{} \left(\rho D \dxi{Z}\right) + \dot{S}_\rho , \label{sm_eq:ZinSpace} \\
\dt{\rho \phi} + \dxi{\rho u_i \phi} &= \frac{1}{\mathrm{Le}_\phi}\dxi{}\left(\rho D \dxi{\phi}\right) + \dot{S}_\rho\phi_l + \dot{\omega}_{\phi}, \label{sm_eq:PhiinSpace}
\end{align}
where  $t$ is the time, $x_i$ and $u_i$ are the spatial coordinate and velocity components in direction $i$, respectively, $\rho$ is the gas phase density, $D$ is the thermal diffusivity, and $\dot{\omega}_{\phi}$ is the chemical source term. The Lewis number of the mixture fraction is set to unity, while $\mathrm{Le}_\phi$ is the Lewis number of the considered scalar. When employing a Lagrangian spray model, the mass source term, $\dot{S}_\rho$, appears due to evaporation. $\phi_l$ denotes the scalar mass fraction in the liquid phase. 
\par
In LES, filtered flow fields are solved. For reactive flows, density-weighted filtering, i.e., Favre filtering, is commonly employed, which can be achieved by integrating the flow variables, e.g., a scalar $\phi$, against a filter kernel, $\mathcal{F}$, according to
\begin{align}
\orho(\mathbf{x},t) \fav{\phi}(\mathbf{x},t) = \ol{\rho(\mathbf{x},t) \phi(\mathbf{x},t)} &= \int_V \mathcal{F}\left(\mathbf{r}\right)\rho(\mathbf{x}+\mathbf{r}) \phi(\mathbf{x}+\mathbf{r})  \mathrm{d}\mathbf{r}, \label{sm_eq:favre_filtering} \\
\orho(\mathbf{x},t) &= \int_V \mathcal{F}\left(\mathbf{r}\right)\rho(\mathbf{x}+\mathbf{r})   \mathrm{d}\mathbf{r}.
\end{align}
To derive the balance equations for the filtered quantities, commutation of filtering and differentiation has to be assumed, which is not universally valid \citeapp{Ghosal1995} but is commonly made \citeapp{Poinsot2005}. Another method exists to obtain the filtered quantities in LES that employs the concept of filtered density functions (FDF). For any function $g(\mathbf{x},t)$, the filtered value can be obtained via 
\begin{equation}
\ol{g(\mathbf{x},t)} = \int_{\boldsymbol{\Psi}} {f}\left(\boldsymbol{\psi};\mathbf{x},t\right)g(\boldsymbol{\psi})  \mathrm{d}\boldsymbol{\psi}, \label{sm_eq:fdf_filteringDef} 
\end{equation}
where $f$ is the joint FDF of all random variables, $\boldsymbol{\psi}$ is the vector of all sample space variables, and $\boldsymbol{\Psi}$ represents the entire sample space. For variable-density flows, it is convenient to solve for density-weighted filtered quantities that can be obtained via 
\begin{equation}
\ol{\rho(\mathbf{x},t)g(\mathbf{x},t)} =  \orho(\mathbf{x},t) \fav{g}(\mathbf{x},t) = \int_{\boldsymbol{\Psi}} {f}\left(\boldsymbol{\psi};\mathbf{x},t\right){\rho}(\boldsymbol{\psi})g(\boldsymbol{\psi})  \mathrm{d}\boldsymbol{\psi}, \label{sm_eq:fdf_filtering} 
\end{equation}
or
\begin{equation}
\fav{g}(\mathbf{x},t) = \int_{\boldsymbol{\Psi}} \fav{f}\left(\boldsymbol{\psi};\mathbf{x},t\right)g(\boldsymbol{\psi})  \mathrm{d}\boldsymbol{\psi}, \label{sm_eq:fdf_Favrefiltering} 
\end{equation}
where $\fav{f}$ denotes the Favre-FDF. Solving for the entire joint FDF is computationally demanding. However, the distribution of a single random variable is often known or can be modeled more easily. In that case, the joint FDF can be split into the marginal FDF of the known variable and the conditional FDF of all others. Hence, considering the case of a turbulent mixing field, where the velocity components and the mixture fraction are randomly distributed, we can write
\begin{equation}
\fav{f}(\psi,\mathbf{v};\mathbf{x},t) = \ff(\psi;\mathbf{x},t) f_{\mathbf{u}|Z}(\mathbf{v}|\psi;\mathbf{x},t),
\end{equation}
where $\ff$ is the marginal density-weighted mixture fraction FDF, for which well-established models exist, and $f_{\mathbf{u}|Z}$ is the velocity distribution given the condition $Z\left(\mathbf{x},t\right)=\psi$. Note that $\psi$ and $\mathbf{v}$ refer to the mixture fraction and velocity sample space variables, respectively. Using this concept, the filtered value of a function that depends on the mixture fractions as well as the velocity field can be obtained via 
\begin{equation}
\fav{g}(\mathbf{x},t) = \int_\Psi \ff(\psi;\mathbf{x},t)\cond{g} \mathrm{d}\mathbf{\psi}, \label{sm_eq:FavreCond}
\end{equation}
where $\cond{g}$ is the conditional expectation that is defined by the integration of $g$ against the conditional FDF over the entire velocity sample space, $\mathbf{V}$,
\begin{equation}
\cond{g}=\int_\mathbf{V} f_{\mathbf{u}|Z}(\mathbf{v}|\psi;\mathbf{x},t)g(\psi,\mathbf{v}) \mathrm{d}\mathbf{v}.
\end{equation}
Applying filtering to Eqs.~(\ref{sm_eq:Continuity})-(\ref{sm_eq:PhiinSpace}) yields the filtered governing equations, which read
\begin{align}
\dt{\orho } + \dxi{\orho \fav{u}_i } &= \ol{\dot{S}}_\rho, \label{sm_eq:ContinuityFil1} \\*
\dt{\orho \fav{Z}} + \dxi{\orho \fav{u_i Z}} &= \dxi{} \left(\orho \fav{D \dxi{Z}}\right) + \ol{\dot{S}}_\rho , \label{sm_eq:ZinSpaceFil1} \\*
\dt{\orho \fav{\phi}} + \dxi{\orho \fav{u_i \phi}} &= \frac{1}{\mathrm{Le}_\phi}\dxi{}\left(\orho \fav{D \dxi{\phi}}\right) + \ol{\dot{S}_\rho\phi_l} + \ol{\dot{\omega}}_{\phi}. \label{sm_eq:PhiinSpaceFil1}
\end{align}
For a given marginal mixture fraction FDF, Eqs.~(\ref{sm_eq:ContinuityFil1})-(\ref{sm_eq:PhiinSpaceFil1}) can be rewritten using Eq.~(\ref{sm_eq:fdf_Favrefiltering}) and Eq.~(\ref{sm_eq:FavreCond}) as
\begin{align}
\int_\Psi \left(\dt{\orho \ff } 	+ \dxi{\orho \ff \cond{u_i}} \right)\mathrm{d}\psi 		
 =& \int_\Psi \orho \ff \cond{\frac{\dot{S}_\rho}{\rho}} \mathrm{d}\psi , \label{sm_eq:ContinuityFil} 
 \\*
\int_\Psi \left(\dt{\orho \ff \psi} + \dxi{\orho \ff \cond{u_i} \psi} \right)\mathrm{d}\psi 	
=& \int_\Psi \left[\dxi{} \left(\orho \ff \cond{D \dxi{Z}}\right) + \orho \ff \cond{\frac{\dot{S}_\rho}{\rho}}\right] \mathrm{d}\psi, \label{sm_eq:ZinSpaceFil} \\*
\int_\Psi \left(\dt{\orho \ff \cond{\phi}} + \dxi{\orho \ff \cond{u_i \phi}}\right) \mathrm{d}\psi		
=& \int_\Psi \left[\frac{1}{\mathrm{Le}_\phi}\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right)  +  \orho \ff \cond{\frac{\dot{S}_\rho\phi_l}{\rho}} + \orho \ff \cond{\frac{\dot{\omega}_{\phi}}{\rho}}\right] \mathrm{d}\psi . \label{sm_eq:PhiinSpaceFil}
\end{align}
\section{Fine-grained FDF concept}\noindent
The concept of the fine-grained PDF allows for convenient manipulation of PDF transport equations \citeapp{Pope2000} in a RANS context. However, the associated methods can be similarly applied to LES and FDF equations. Since this paper focuses on mixture fraction based combustion models, we consider the mixture fraction FDF exclusively.
The fine-grained FDF is defined using the Dirac delta function as
\begin{equation}
\fg = \delta\left[\psi-Z(x,t)\right], \label{sm_eq:fineGrainedDef}
\end{equation}
where $\psi$ is the mixture fraction sample variable. To make use of the fine-grained FDF in the following, some important properties of the Dirac delta function need to be presented first.
\subsection{Properties of the Dirac delta function}\noindent
This section briefly summarizes some properties of the Dirac delta function that are useful for the following model derivation. For a more detailed description of the Dirac delta function, the reader is referred to the textbook of Pope \citeapp{Pope2000}. The Dirac delta function is defined as follows
\begin{align}
\delta(x) &=
    \begin{cases}
       \infty, &x=0 \\
        0, &\text{elsewhere},
    \end{cases} \label{sm_eq:DiracDef1}
    \\
    \int_{-\infty}^\infty \delta(x)\mathrm{d}x &= 1. \label{sm_eq:DiracDef2}
\end{align}
Some basic properties of the Dirac delta functions are:
\begin{enumerate}
\item The Dirac delta function is symmetric 
\begin{equation}
\delta(x-a)=\delta(a-x) \label{sm_eq:Dirac1}
\end{equation}
\item For any continuous function $g(x)$ and $\Delta x>0$ it holds that
\begin{equation}
\int_{a-\frac{\Delta x}{2}}^{a+\frac{\Delta x}{2}} \delta(x-a)g(x)\mathrm{d}x = g(a). \label{sm_eq:Dirac2}
\end{equation}
\item Furthermore, the following equation holds:
\begin{equation}
\delta(x-a)g(x)=\delta(x-a)g(a)  \label{sm_eq:Dirac3}
\end{equation}
\item The derivative of the Dirac delta function, $\delta'$, is not explicitly defined. However, one can find a relation for the product of the delta function derivative and any continuous function by integrating Eq.~(\ref{sm_eq:Dirac2}) by parts as 
\begin{equation}
\int_{a-\frac{\Delta x}{2}}^{a+\frac{\Delta x}{2}} \delta'(x-a)g(x)\mathrm{d}x = \left[\delta(x-a)g(x) \right]_{a-\frac{\Delta x}{2}}^{a+\frac{\Delta x}{2}} -\int_{a-\frac{\Delta x}{2}}^{a+\frac{\Delta x}{2}} \delta(x-a)g'(x)\mathrm{d}x.  \label{sm_eq:DiracDiff1}
\end{equation}
The first term on the right-hand side vanishes due to Eq.~(\ref{sm_eq:DiracDef1}), and hence,
\begin{equation}
\int_{a-\frac{\Delta x}{2}}^{a+\frac{\Delta x}{2}} \delta'(x-a)g(x)\mathrm{d}x = -g'(a). \label{sm_eq:DiracDiff2}
\end{equation}
\item
Furthermore, Eq.~(\ref{sm_eq:DiracDiff1}) holds for infinitesimally small $\Delta x$, and thus, it follows from the main theorem of calculus that
\begin{equation}
\delta'(x-a)g(x)= -\delta(x-a)g'(x). \label{sm_eq:DiracDiff3}
\end{equation}
\end{enumerate}
\subsection{Properties of the fine-grained FDF}\noindent
The properties of the fine-grained FDF can be analogously derived to those of the fine-grained PDF performed by Pope \citeapp{Pope2000}:
\begin{enumerate}
\item The first important property can be obtained by employing Eq.~(\ref{sm_eq:fdf_filteringDef}) and replacing the integration variable $\psi =\psi'$ and substitution of $g(x)=\delta\left[\psi'-\psi\right]$. Additional invoking of Eq.~(\ref{sm_eq:Dirac2}) yields
\begin{equation}
\ol{\fg}({\psi};\mathbf{x},t) = \int_{{\Psi'}} \delta\left(\psi'-\psi\right)  f_Z({\psi'};\mathbf{x},t)  \mathrm{d}{\psi'} = f_Z({\psi};\mathbf{x},t)  .
\end{equation}
Note that $\Psi'$ refers to the entire mixture fraction sample space. Similarly, one can derive a relation for the Favre-FDF using Eq.~(\ref{sm_eq:fdf_filtering}), which reads
\begin{equation}
\begin{split}
\ol{\rho(\mathbf{x},t) \fg({\psi};\mathbf{x},t)} 	
&= \orho(\mathbf{x},t) \int_{{\Psi'}} \delta\left(\psi'-\psi\right)   \ff({\psi'};\mathbf{x},t)  \mathrm{d}{\psi'} \\
&= \orho(\mathbf{x},t) \ff(\psi;\mathbf{x},t). \label{sm_eq:FineGrained1}
\end{split}
\end{equation}
\item The second important property can be derived for the filtered product of a scalar, $\phi$,  and the fine-grained FDF
\begin{align}
\ol{\rho(\mathbf{x},t) \fg({\psi};\mathbf{x},t) \phi(\mathbf{x},t)} 
=& \orho(\mathbf{x},t) \int_{\Phi} \int_{{{\Psi'}}} \varphi \delta\left(\psi'-\psi\right) \fav{f}_{Z,\phi} (\psi',\varphi ;\mathbf{x},t) \mathrm{d}{{\psi'}}\mathrm{d}{{\varphi}} \notag \\
=& \orho(\mathbf{x},t) \int_{\Phi} \varphi  \fav{f}_{Z,\phi}  (\psi,\varphi ;\mathbf{x},t) \mathrm{d}{\varphi},
\end{align}
where $\fav{f}_{Z,\phi}$ is the joint Favre-FDF of $Z$ and $\phi$, which can be expressed by the marginal mixture fraction Favre-FDF and the conditional scalar FDF, $f_{\phi|Z}$ yielding
\begin{align}
\ol{\rho(\mathbf{x},t) \fg({\psi};\mathbf{x},t) \phi(\mathbf{x},t)} 
=& \orho(\mathbf{x},t) \ff({\psi};\mathbf{x},t) \int_{\Phi} \varphi  f_{\phi|Z}  (\varphi ;\mathbf{x},t) \mathrm{d}{\varphi} \notag \\
=& \orho(\mathbf{x},t) \ff({\psi};\mathbf{x},t) \cond{\phi(\mathbf{x},t)}. \label{sm_eq:FineGrained2}
\end{align} 
\item The temporal and spatial derivatives of the fine-grained FDF can be obtained by invoking the chain rule and read
\begin{align}
\dt{\fg} &= -\delta'[\psi - Z(\mathbf{x},t) ]\dt{Z} = -\dPsi{\fg}\dt{Z} = -\dPsi{}\left[\fg({\psi};\mathbf{x},t) \dt{Z}\right], \label{sm_eq:dtFG} \\*
\dxi{\fg} &= -\delta'[\psi - Z(\mathbf{x},t) ]\dxi{Z} = -\dPsi{\fg}\dxi{Z} = -\dPsi{}\left[\fg({\psi};\mathbf{x},t) \dxi{Z}\right] \label{sm_eq:dxiFG}.
\end{align}
Note that the last step in Eq.~(\ref{sm_eq:dtFG}) and Eq.(\ref{sm_eq:dxiFG}) are valid since $\dt{Z}$ and $\dxi{Z}$ are independent of mixture fraction sample space.
\item Another important property is that
\begin{equation}
\fg\dxi{g(Z)} = \dxi{\fg g(Z)} \label{sm_eq:FGprop}, 
\end{equation}
which easily can be shown using previously introduced properties. First, using Eq.~(\ref{sm_eq:dxiFG}) yields
\begin{equation}
g(Z)\dxi{\fg} = -\dxi{Z} \dPsi{g(Z) \fg}.
\end{equation}
The sifting property of the Dirac delta function (Eq.~(\ref{sm_eq:Dirac3})) then yields
\begin{equation}
g(Z)\dxi{\fg} = -\dxi{Z} \dPsi{ g(\psi) \fg}.
\end{equation}
Applying chain-rule and Eq.~(\ref{sm_eq:DiracDiff3}) results in
\begin{equation}
\begin{split}
g(Z)\dxi{\fg} 	&= -\dxi{Z} \left(\dPsi{ g(\psi)} \fg +  g(\psi) \dPsi{\fg} \right) \\
			&=  -\dxi{Z} \left(\dPsi{ g(\psi)} \fg -  \dPsi{ g(\psi)} \fg \right) = 0.
\end{split}
\end{equation}
\end{enumerate}
\section{Turbulent spray flamelet equation}\noindent
In unsteady non-premixed flamelet models, the reactive scalar is assumed to depend solely on mixture fraction and time. Based on this assumption, the flamelet transformation rules are given as
\begin{align}
\dt{\phi} &\approx \dtau{\hat{\phi}}+ \dt{Z}\dZ{\hat{\phi}}\label{sm_eq:transformation1},\\*
\dxi{\phi} &\approx \dxi{Z}\dZ{\hat{\phi}}. \label{sm_eq:transformation2}
\end{align}
Note that $\dtau{}$ denotes the temporal change at constant mixture fraction, i.e., $\dtau{}=\dt{}\Big|_{Z=const.}$, while $\dt{}$ refers to the partial time derivative at a fixed point in physical space. Furthermore, the hat symbol marks quantities defined in mixture fraction space. %, which are independent of the location in physical space, i.e., 
%\begin{equation}
%\dxi{\hat{\phi}}=0. \label{sm_eq:flameletAssumption}
%\end{equation}
Since the reactive scalar is assumed to be solely dependent on mixture fraction, no conditional scalar fluctuations are present, i.e., $\hat{\phi}=\cond{{\phi}}$. Hence, the conditional scalar expectations in Eq.~(\ref{sm_eq:PhiinSpaceFil}) can be replaced accordingly. Furthermore, we assume the scalar mass fraction inside the liquid phase is constant.
In low Mach number flows, the reaction source term depends solely on the reactive scalars (species and temperature) and the thermodynamic background pressure. Then, the conditional reaction source term in Eq.~(\ref{sm_eq:PhiinSpaceFil}) can be expressed as $\cond{\frac{\dot{\omega}_{\phi}}{\rho}}=\frac{\hat{\dot{\omega}}_{\phi}(\psi,t)}{\hat{\rho}(\psi,t)}$. Note that when Mach numbers become large, compressibility effects additionally influence the local density and temperature, and herewith, the chemical source term. For internal combustion engine flows, high Mach numbers are typically present in the valve gap during gas exchange and close to the injector orifice during fuel injection. However, the Mach numbers are usually small in regions where combustion takes place. Hence, the compressibility effects on the chemical source terms are neglected in this work. Consequently, Eq.~(\ref{sm_eq:PhiinSpaceFil}) can be reformulated using the assumptions as mentioned above and differentiating both sides with respect to $\psi$ as
%\begin{equation}
%\dt{\orho \ff \hat{\phi}} + \dxi{\orho \ff \cond{u_i} \hat{\phi}} 	
%=  \frac{1}{\mathrm{Le}_\phi}\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right)  +  \orho \ff \cond{\frac{\dot{S}_\rho}{\rho}}\phi_l + \orho \ff \frac{\hat{\dot{\omega}}_{\phi}}{\hat{\rho}}. \label{sm_eq:PhiinSpaceFlamelet}
%\end{equation}
\begin{equation}
\dt{\orho \ff \cond{\phi}} + \dxi{\orho \ff \cond{u_i \phi}} 	
=  \frac{1}{\mathrm{Le}_\phi}\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right)  +  \orho \ff \cond{\frac{\dot{S}_\rho}{\rho}}\phi_l + \orho \ff \frac{\hat{\dot{\omega}}_{\phi}}{\hat{\rho}}. \label{sm_eq:PhiinSpaceFlamelet}
\end{equation}
In the following, Eq.~(\ref{sm_eq:PhiinSpaceFlamelet}) will be transformed into mixture fraction sample space, which, however, requires some mathematical transformations using the fine-grained FDF concept. Invoking the first two properties of the fine-grained FDF (Eq.~(\ref{sm_eq:FineGrained1}) and Eq.~(\ref{sm_eq:FineGrained2})), the left-hand side of Eq.~(\ref{sm_eq:PhiinSpaceFlamelet}) can be written as
\begin{align}
\dt{\orho \ff \cond{\phi}} + \dxi{\orho \ff \cond{u_i \phi}} 	= \ol{\dt{\rho\fg\hat{\phi}} + \dxi{\rho u_i \fg \hat{\phi}}}.
\end{align}
Applying the product rule and invoking continuity (Eq.~(\ref{sm_eq:Continuity})) yield
\begin{equation}
\ol{\dt{\rho\fg\hat{\phi}} + \dxi{\rho u_i \fg \hat{\phi}}} =
 \ol{\hat{\phi} \left(\rho\dt{\fg}  
 + \rho u_i\dxi{\fg}
 +\fg \dot{S}_\rho \right)
 +\rho \fg \left(\dtau{\hat{\phi}}+u_i\dxi{\hat{\phi}}\right)}. \label{sm_eq:pdf_transport_nc1}
\end{equation}
The substantial derivative of the FDF can be expressed using Eq.~(\ref{sm_eq:dtFG}) and Eq.~(\ref{sm_eq:dxiFG}) as $
\dt{\fg}+u_i \dxi{\fg} = -\dPsi{\fg}\left(\dt{Z}+ u_i \dxi{Z}\right)$ yielding
\begin{align}
\ol{\dt{\rho\fg\hat{\phi}} + \dxi{\rho u_i \fg \hat{\phi}}} = 
\ol{-\hat{\phi}\dPsi{\fg}\left(\rho \dt{Z}
+\rho u_i \dxi{Z}\right)
+\rho \fg \left(\dtau{\hat{\phi}}+u_i\dxi{\hat{\phi}}\right) 
+\fg \dot{S}_\rho \hat{\phi}}.
\end{align}
From Eq.~(\ref{sm_eq:DiracDiff3}) follows $\dPsi{\fg}\hat{\phi}=-\fg\dPsi{\hat{\phi}}$.
Additionally, Eq.~(\ref{sm_eq:ZinSpace}) can be inserted in non-conservative form, yielding
\begin{equation}
\ol{\dt{\rho\fg\hat{\phi}} + \dxi{\rho u_i \fg \hat{\phi}}} = 
\ol{\left[\rho \fg \dxi{} \left(\rho D \dxi{Z}\right) 
+ \fg \dot{S}_\rho (1-\psi)\right] \dPsi{\hat{\phi}} 
+ \fg \dot{S}_\rho \hat{\phi}
+ \rho \fg \left(\dtau{\hat{\phi}}+u_i\dxi{\hat{\phi}}\right)}. \label{sm_eq:CondPhiLHS}
\end{equation}
Eq.~(\ref{sm_eq:CondPhiLHS}) can now be transformed back to an FDF formulation using Eq.~(\ref{sm_eq:FineGrained1}) and Eq.~(\ref{sm_eq:FineGrained2}) yielding the transformed left-hand side of Eq.~(\ref{sm_eq:PhiinSpaceFlamelet})
\begin{equation}
\begin{split}
&\dt{\orho\ff\hat{\phi}} + \dxi{\orho \cond{u_i} \ff \hat{\phi}} = 
\orho \ff \left\{\left[ \cond{\frac{1}{\rho}\dxi{}\left(\rho D \dxi{Z}\right)} 
+ \cond{\frac{\dot{S}_\rho}{\rho}} (1-\psi)\right] \dPsi{\hat{\phi}} 
+  \cond{\frac{\dot{S}_\rho}{\rho}} \hat{\phi}
+  \left(\dtau{\hat{\phi}}+\cond{u_i}\dxi{\hat{\phi}}\right)\right\}. 
\label{sm_eq:CondPhiLHSfinal}
\end{split}
\end{equation}
For transforming the right-hand side of Eq.~(\ref{sm_eq:PhiinSpaceFlamelet}), particular focus must be directed toward the diffusion term, while no further manipulation of the source terms is required.
The diffusion term can be manipulated by using the fine-grained FDF concept, i.e., using again Eq.~(\ref{sm_eq:FineGrained1}) and Eq.~(\ref{sm_eq:FineGrained2}), and invoking the flamelet transformation (Eq.~(\ref{sm_eq:transformation2})) yielding
\begin{equation}
\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right) = \ol{\dxi{}\left(\rho \fg D \dxi{Z} \dZ{\hat{\phi}}\right)}.
\end{equation}
Invoking the sifting property of $\fg$ (Eq.~(\ref{sm_eq:Dirac3})), we can write $\fg\dZ{\hat{\phi}}=\fg\dPsi{\hat{\phi}}$, which then can be expressed using Eq.~(\ref{sm_eq:DiracDiff3}) as $\fg\dPsi{\hat{\phi}}=-\dPsi{\fg}\hat{\phi}$. 
%Additionally, we use the flamelet assumption (Eq.~(\ref{sm_eq:flameletAssumption})) to obtain
\begin{equation}
\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right) = -\ol{\dxi{\hat{\phi}}\left(\rho D \dxi{Z} \dPsi{\fg}\right)} -\ol{\hat{\phi}\left[\dxi{}\left(\rho D \dxi{Z} \dPsi{\fg}\right)\right]}. 
\end{equation}
Note that the term $\rho D \dxi{Z}$ is independent of $\psi$, and hence, the order of differentiation can be altered as
\begin{equation}
\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right) = -\ol{\dxi{\hat{\phi}}\dPsi{}\left(\rho D \dxi{Z} \fg\right)} -\ol{\hat{\phi}\dPsi{}\left[\dxi{}\left(\rho D \dxi{Z} \fg\right)\right]}. \label{sm_eq:diffterm}
\end{equation}
The second term on the right-hand side of Eq.~(\ref{sm_eq:diffterm}) can be reformulated using the product rule for the spatial derivative and inserting Eq.~(\ref{sm_eq:dxiFG}), yielding
\begin{equation}
\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right) = -\ol{\dxi{\hat{\phi}}\dPsi{}\left(\rho D \dxi{Z} \fg\right)} + \ol{\hat{\phi}\ddPsi{\fg}\left(\rho D \dxi{Z}\dxi{Z}\right)} 
- \ol{\hat{\phi} \dPsi{\fg} \dxi{}\left(\rho D \dxi{Z} \right)}.
\end{equation}
From Eq.~(\ref{sm_eq:DiracDiff3}) follows $-\dPsi{\fg}\hat{\phi}=\fg\dPsi{\hat{\phi}}$ and $\ddPsi{\fg}\hat{\phi}=\fg\ddPsi{\hat{\phi}}$. Finally, the diffusion term can be expressed using the FDF formulation by invoking Eq.~(\ref{sm_eq:FineGrained1}) and Eq.~(\ref{sm_eq:FineGrained2}) as 
\begin{equation}
\dxi{}\left(\orho \ff \cond{D \dxi{\phi}}\right) = -\dxi{\hat{\phi}}\dPsi{}\left(\orho\ff \cond{D \dxi{Z}} \right) + \orho \ff \cond{D \dxi{Z}\dxi{Z}} \ddPsi{\hat{\phi}}
+\orho \ff  \cond{\frac{1}{\rho}\dxi{}\left(\rho D \dxi{Z} \right)} \dPsi{\hat{\phi}}.  \label{sm_eq:CondPhiRHS}
\end{equation}
Eqs.~(\ref{sm_eq:CondPhiLHS}) and (\ref{sm_eq:CondPhiRHS}) can be combined to obtain the local non-premixed turbulent flamelet equation
\begin{equation}
\begin{split}
\orho \ff \dtau{\hat{\phi}} + 
\orho \ff \left[\cond{\xi_Z} \left(1 - \frac{1}{\mathrm{Le}_\phi} \right) + \cond{\zeta_Z}\left(1-\psi\right)\right] &\dPsi{\hat{\phi}} + \orho\ff\cond{\eta_Z} \dxi{\hat{\phi}}= \\
&  \frac{\orho \ff}{2 \mathrm{Le}_\phi} \cond{\chi_Z} \ddPsi{\hat{\phi}} 
+ \orho\ff \cond{\zeta_Z} \left( \phi_l - \hat{\phi}\right)
+ \orho \ff \frac{\hat{\dot{\omega}}_{\phi}}{\hat{\rho}}. 
\end{split}\label{sm_eq:flamelet_local}
\end{equation}
where the conditional flow parameters, conditional mixture fraction dissipation rate, $\cond{\chi_Z}$, conditional mixture fraction diffusion rate, $\cond{\xi_Z}$, conditional velocity, $\cond{\eta_Z}$, and conditional normalized mass source, $\cond{\zeta_Z}$, have been introduced, which are defined as
\begin{align}
\cond{\chi_Z} 	&= 2\cond{D \dxi{Z}\dxi{Z}}, \\*
\cond{\xi_Z} 	&= \cond{\frac{1}{\rho}\dxi{}\left(\rho D \dxi{Z} \right)}, \\*
\cond{\eta_Z} 	&= \cond{u_i} + \frac{1}{\orho\ff}\dPsi{}\left(\orho\ff \cond{D\dxi{Z}}\right), \\*
\cond{\zeta_Z} 	&=\cond{\frac{\dot{S}_\rho}{\rho}}.
\end{align}
Note that the spatial convection term vanishes since $\hat{\phi}$ is a function of $Z$ and $\tau$, and thus, is independent of space, i.e. $\dxi{\hat{\phi}}=0$. Consequently, $\hat{\phi}$ represents a global solution. The evolution of the $\hat{\phi}$ can be obtained by integrating Eq.~(\ref{sm_eq:flamelet_local}) over the entire system volume $\Omega$. An FDF-independent equation can be obtained by dividing by $\int_\Omega\orho \ff\mathrm{d}V$
\begin{equation}
 \dtau{\hat{\phi}} + 
 \left[\xi_G \left(1 - \frac{1}{\mathrm{Le}_\phi} \right) 
       + \zeta_G\left(1-\psi\right)\right] \dPsi{\hat{\phi}} =  \frac{1}{2 \mathrm{Le}_\phi} 
   \chi_G \ddPsi{\hat{\phi}} 
+ \zeta_G \left( \phi_l - \hat{\phi}\right)
+ \frac{\hat{\dot{\omega}}_{\phi}}{\hat{\rho}}, \label{sm_eq:turb_spray_flamelet}
\end{equation}
where the global conditional flow parameters are defined as
\begin{align}
\chi_G &=\frac{\int \orho \ff \cond{\chi_Z}\mathrm{d}V}{\int \orho \ff \mathrm{d}V}, 	\label{sm_eq:globalChi}\\*
\xi_G &= \frac{\int \orho \ff \cond{\xi_Z}\mathrm{d}V}{\int \orho \ff \mathrm{d}V} ,		\label{sm_eq:globalXi}\\*
\zeta_G &= \frac{\int \orho \ff \cond{\zeta_Z}\mathrm{d}V}{\int \orho \ff \mathrm{d}V}. \label{sm_eq:globalZeta}
\end{align}
Note that Eq~(\ref{sm_eq:turb_spray_flamelet}) is the classical flamelet equation, which is formulated in non-conservative form, and furthermore, it should be noted that the turbulent flamelet equation is only defined for sample space locations with $\int_\Omega \orho \ff \mathrm{d}V > 0$. Eq.~(\ref{sm_eq:flamelet_local}) could also be formulated in conservative form, which, however, is not independent of $\ff$. 
\section{Consistent mixing model}\noindent
Solving the global flamelet equation (Eq.~(\ref{sm_eq:turb_spray_flamelet})) requires knowledge of the global conditional flow parameters.  
It should be noted that the conditional flow parameters are linked to the mixture evolution, i.e., transport in mixture fraction space is related to mixture fraction transport in physical space. Modeling the flow parameters independently of the mixture evolution results in scalar mass conservation errors. The global conditional dissipation and diffusion rate can be formulated consistently from the global mixture evolution for single-phase flows in closed systems \citeapp{Davidovic2022}. For other systems, the local parameters need to be expressed consistently to the local FDF evolution first. The global parameters can then be obtained from Eq.~(\ref{sm_eq:globalChi})-Eq.~(\ref{sm_eq:globalZeta}). The derivation of the local consistent flow parameters is described in this section.
\subsection{Mixture fraction FDF transport equation}\noindent
The mixture fraction FDF transport equation can be derived from the governing equations using the fine-grained FDF concept. Following the procedure described by Pope \citeapp{Pope2000}, the mixture fraction FDF transport in evaporative flows reads
\begin{equation}
\orho\dt{\ff}+\orho \fav{u}_i \dxi{\ff} = 
-\dPsi{\orho\ff \cond{\xi_Z}} 
- \dxi{\orho \left(\cond{u_i} - \fav{u}_i\right) \ff} 
- \dPsi{}\left[\orho\ff\cond{\zeta_Z}(1-\psi)\right]
+\ff \left(\orho \cond{\zeta_Z}-\ol{\dot{S}}_\rho\right). \label{sm_eq:FDFtransportExact}
\end{equation}
Note that an exact relation exists between the conditional diffusion and dissipation rate that can be derived using the fine-grained FDF and reads
\begin{equation}
-\dPsi{\orho\ff \cond{\xi_Z}} =  \dxi{}\left(\ol{\rho D\dxi{\fg}}\right) - \frac{1}{2}\ddPsi{\orho\ff\cond{\chi_Z}}. \label{sm_eq:condDiffcondDiss1}
\end{equation}
The first term on the right-hand side in Eq.~(\ref{sm_eq:condDiffcondDiss1}) requires modeling in case of space-variant $\rho D$ since
\begin{equation}
\begin{split}
 \dxi{}\left(\ol{\rho D\dxi{\fg}}\right) 	&= \dxi{}\left(\dxi{\ol{\rho \fg D}}\right)-\dxi{}\left(\ol{\fg\dxi{\rho D}}\right) 
 						    	= \dxi{}\left(\dxi{\orho \ff \fav{D}}\right)-\dxi{}\left(\orho\ff\cond{\frac{1}{\rho}\dxi{\rho D}}\right) \\
							&= \dxi{}\left(\orho \fav{D}\dxi{\ff}\right)+\dxi{}\left[\ff\left(\dxi{\orho \fav{D}}-\orho\cond{\frac{1}{\rho}\dxi{\rho D}}\right)\right]. \label{sm_eq:lam_assumption1}
\end{split}
\end{equation}
A common model is to assume that 
\begin{equation}
\left(\dxi{\orho \fav{D}}-\orho\cond{\frac{1}{\rho}\dxi{\rho D}}\right)\approx0,\label{sm_eq:lam_assumption}
\end{equation}
yielding the relation between $\cond{\chi_Z}$ and $\cond{\xi_Z}$ as
\begin{equation}
\dPsi{\orho\ff \cond{\xi_Z}} =  \frac{1}{2}\ddPsi{\orho\ff\cond{\chi_Z}} - \dxi{}\left(\orho \fav{D}\dxi{\ff}\right). \label{sm_eq:condDiffcondDiss2}
\end{equation}
Furthermore, we approximate the subfilter FDF fluxes using a gradient transport approach defined as
\begin{equation}
 \left(\cond{u_i} - \fav{u}_i\right) \ff = - D_{t,\psi} \dxi{\ff} \label{sm_eq:ff_grad_assumption}.
\end{equation}
Note that the eddy diffusivity $D_{t,\psi}$ is a function of $\psi$ and $\textbf{x}$ and $t$.
Inserting Eq.~(\ref{sm_eq:condDiffcondDiss2}) and Eq.~(\ref{sm_eq:ff_grad_assumption}) into Eq.~(\ref{sm_eq:FDFtransportExact}) relates the FDF evolution to the conditional mixture fraction diffusion rate and conditional spray source term 
\begin{equation}
\orho\dt{\ff}+\orho \fav{u}_i \dxi{\ff} =
 - \frac{1}{2}\ddPsi{\orho\ff\cond{\chi_Z}} 
+ \dxi{}\left[\orho \left(\fav{D} + {D}_{t,\psi}\right) \dxi{\ff}\right] 
-  \dPsi{}\left[\orho\ff\cond{\zeta_Z}(1-\psi)\right] 
+\ff \left(\orho \cond{\zeta_Z}-\ol{\dot{S}}_\rho\right). \label{sm_eq:pdf_trans_chi}
\end{equation}
%Note that $\cond{\xi_Z}$ can be obtained from Eq.~(\ref{sm_eq:condDiffcondDiss2}), once $\cond{\chi_Z}$ is known.
Eq.~(\ref{sm_eq:pdf_trans_chi}) can be used to solve for $\ff$ given models for $\cond{\chi_Z}$ and $\cond{\zeta_Z}$. This approach enforces consistent mixing in physical and flamelet space. However, solving for $\ff$ is expensive, and more importantly, good models exist for predicting subfilter mixing of conserved scalars. Hence, in this work, we aim to prescribe the FDF evolution using the presumed FDF approach and obtain the associated conditional flow parameters from Eq.~(\ref{sm_eq:condDiffcondDiss2}) and Eq.~(\ref{sm_eq:pdf_trans_chi}). 
The presumed FDF approach prescribes a functional form of the FDF, which is parameterized by its statistical moments. The statistical moments are then solved in physical space using modeled transport equations. 
The beta distribution is most commonly used to model the turbulent mixing of conserved scalars. For flows with evaporation, the maximum mixture fraction is typically substantially below unity due to saturation effects. The distribution function should ensure a proper definition in $\Zmin < Z < \Zmax$. For those cases, a modified beta distribution has been suggested in previous studies \citeapp{Reveillon2000}\citeapp{Ge2006}, which reads
\begin{equation}
\ff =
    \begin{cases}
        \frac{1}{B(a,b)\Delta Z}{\psi^*}^{a-1} \left(1-\psi^*\right)^{b-1} & \text{if } 0 < \psi^* < 1,\\
        0 & \text{elsewhere }.
    \end{cases} \label{sm_eq:scaledBeta}
\end{equation}
with $\psi^*=\left(\psi-\Zmin\right)/\Delta Z$ and $\Delta Z=\Zmax-\Zmin$. $B(a,b)$ is the beta function, which is defined as $B(a,b)=\int_0^1 {x}^{a-1} \left(1-x\right)^{b-1}\mathrm{d}x$ and is related to the gamma function via ${B(a,b)=\Gamma(a)\Gamma(b)/\Gamma(a+b)}$.
The shape parameters are computed such that the distribution resembles the first and second mixture fraction moment
\begin{align}
a &=  \frac{\fav{Z}-\Zmin}{\Delta Z}\left[\frac{\left(\fav{Z}-\Zmin\right) \left(\Zmax - \fav{Z}\right)}{\fav{Z^2}-\fav{Z}^2} - 1\right],  \\*
b &= \frac{\Zmax-\fav{Z}}{\Delta Z}\left[\frac{\left(\fav{Z}-\Zmin\right) \left(\Zmax - \fav{Z}\right)}{\fav{Z^2}-\fav{Z}^2} - 1\right].
\end{align}
A-priori analyses have shown that the rescaled beta function is a good approximation for turbulent evaporative flows when space-variant mixture fraction limits, denoted here as $\Zmin$ and $\Zmax$, are employed \citeapp{Ge2006}\citeapp{Luo2011}. Thus, the temporal and spatial FDF derivatives can be approximated as
\begin{align}
\dt{\ff} &= \dt{\fav{Z}}\frac{\partial\ff}{\partial \fav{Z}} + \dt{\fav{Z^2}}\frac{\partial\ff}{\partial \fav{Z^2}} 
+ \dt{\Zmin}\frac{\partial\ff}{\partial{\Zmin}} +  \dt{\Zmax}\frac{\partial\ff}{\partial {\Zmax}} \label{sm_eq:dFDFdt}, \\*
\dxi{\ff} &= \dxi{\fav{Z}}\frac{\partial\ff}{\partial \fav{Z}} + \dxi{\fav{Z^2}}\frac{\partial\ff}{\partial \fav{Z^2}} 
+ \dxi{\Zmin}\frac{\partial\ff}{\partial {\Zmin}} +  \dxi{\Zmax}\frac{\partial\ff}{\partial {\Zmax}}  \label{sm_eq:dFDFdxi}.
\end{align}
However, models for the spatial evolution of $\Zmin$ and $\Zmax$ do not yet exist, and thus, space-invariant values are employed in the present study. For the minimum mixture fraction, $\Zmin=0$ is used. For modeling $\Zmax$, it is assumed that the FDF is strongly negatively skewed for large $\fav{Z}$, and hence 
\begin{equation}
\Zmax(t) \approx \max_{\substack{\textbf{x}\in\Omega \\ t^*\leq t}} \left[\fav{Z}(\textbf{x},t^*)\right].
\end{equation}
$\Zmax$ ramps up after start-of-injection (SOI) and remains constant after reaching its maximum value, i.e., $\Zmax$ exhibits a substantial temporal change in the beginning, which rapidly decays. Thus, $\dt{\Zmax}$ is expected to be small in regions where combustion takes place, and hence, Eqs.~(\ref{sm_eq:dFDFdt}) and (\ref{sm_eq:dFDFdxi}) simplify to
\begin{align}
\dt{\ff} &= \dt{\fav{Z}}\frac{\partial\ff}{\partial \fav{Z}} + \dt{\fav{Z^2}}\frac{\partial\ff}{\partial \fav{Z^2}}, \label{sm_eq:dFDFdtmodel} \\
\dxi{\ff} &= \dxi{\fav{Z}}\frac{\partial\ff}{\partial \fav{Z}} + \dxi{\fav{Z^2}}\frac{\partial\ff}{\partial \fav{Z^2}}. \label{sm_eq:dFDFdximodel}
\end{align}
The mixture fraction moment transport equations can be derived from Eqs.~(\ref{sm_eq:Continuity}), (\ref{sm_eq:ZinSpace}), and (\ref{sm_eq:favre_filtering}) and read
\begin{align}
\orho\dt{ \fav{Z}} + \orho \fav{u}_i \dxi{ \fav{Z}} = &
\dxi{}\left(\ol{\rho D\dxi{Z}}\right) 
- \dxi{}\left(\orho\fav{u_i Z} - \orho\fav{u}_i\fav{Z}\right) + \ol{\dot{S}}_\rho \left(1-\fav{Z}\right),
\label{sm_eq:Z1trans}\\ 
\label{sm_eq:Z2trans}
\orho\dt{ \fav{Z^2}} + \orho \fav{u}_i \dxi{ \fav{Z^2}} =& 
\dxi{}\left(\ol{\rho D\dxi{Z^2}}\right)
-\dxi{}\left(\orho\fav{u_i Z^2} - \orho\fav{u}_i\fav{Z^2}\right) - \orho\fav{\chi}_Z+ \ol{\dot{S}_\rho \left(2Z-Z^2\right)} - \ol{\dot{S}}_\rho\fav{Z^2}.  
\end{align}
Note that the subfilter moment fluxes need to be formulated consistently to the subfilter FDF fluxes. The consistency requirements for the filtered laminar diffusion fluxes and the turbulent subfilter fluxes are presented in the following. 
\subsubsection{Consistent filtered laminar diffusion fluxes}
The filtered laminar diffusion flux of the $\mathrm{n^{th}}$ mixture fraction moment can be written using the FDF as
\begin{align}
\ol{\rho D \dxi{Z^n} }
&=  \int_\Psi \orho\ff \cond{D\dxi{Z^n}}  \mathrm{d}\psi =  \int_\Psi \ol{\rho\fg D\dxi{Z^n}},  \label{sm_eq:lamMomFlux1}
\end{align}
where the fine-grained FDF concept (Eqs.~(\ref{sm_eq:FineGrained1}) and (\ref{sm_eq:FineGrained2})) has been applied to obtain the second step in Eq.~(\ref{sm_eq:lamMomFlux1}). 
Invoking the properties of the fine-grained FDF (Eqs.~(\ref{sm_eq:FGprop}) (\ref{sm_eq:Dirac3})) then yields
\begin{align}
\ol{\rho D \dxi{Z^n} }
&=  \int_\Psi \dxi{}\left(\ol{\rho D\dxi{\fg\psi^n}}\right) \mathrm{d}\psi. \label{sm_eq:lamMomFlux2}
\end{align}
Eq.~(\ref{sm_eq:lamMomFlux2}) can manipulated in the same way as Eq.~(\ref{sm_eq:lam_assumption1}) resulting in
\begin{align}
\ol{\rho D \dxi{Z^n} }
&= \int_\Psi \orho \fav{D} \psi^n \dxi{\ff}+ \psi^n \ff \left(\dxi{\orho \fav{D}}-\orho \cond{\frac{1}{\rho}\dxi{\rho D}}\right) \mathrm{d}\psi, \label{sm_eq:lamMomFlux3}
\end{align}
which shows that the same unclosed term appears in both the filtered laminar moment flux equations and the filtered laminar FDF flux equation. In the present work, Eq.~(\ref{sm_eq:lam_assumption}) is used to close the filtered laminar diffusion fluxes. However, it should be noted that any model could be used as long as the same is applied in Eq.~(\ref{sm_eq:lam_assumption1}) and Eq.~(\ref{sm_eq:lamMomFlux3}).
\subsubsection{Consistent turbulent subfilter fluxes}
For closing the turbulent subfilter moment fluxes consistently to the subfilter mixture evolution, a consistency condition can be derived by expressing the moment fluxes using the FDF as
\begin{align}
 \left(\fav{u_i Z^n} - \fav{u}_i\fav{Z^n}\right) 
&=  \int_\Psi \left(\cond{u_i} - \fav{u}_i\right) \ff \psi^n \mathrm{d}\psi. \label{sm_eq:sgs_flux1}
\end{align}
The same unclosed term appears in both the subfilter moment and FDF fluxes. Hence, a consistent transport modeling approach requires the same closure for $\left(\cond{u_i} - \fav{u}_i\right) \ff$ in Eq.~(\ref{sm_eq:FDFtransportExact}) and Eq.~(\ref{sm_eq:sgs_flux1}). However, the turbulent subfilter moment fluxes are commonly modeled independently of the conditional flow parameters and the herewith associated FDF evolution. Note that the condition in Eq.~(\ref{sm_eq:sgs_flux1}) needs to be satisfied regardless of the subfilter model type. However, in the following, we will focus on Smagorinsky-type models because of their widespread use. If a Smagorinsky-type model is employed, Eq.~(\ref{sm_eq:sgs_flux1}) can be rewritten using Eq.~(\ref{sm_eq:ff_grad_assumption}) as
\begin{equation}
 \left(\fav{u_i Z^n} - \fav{u}_i\fav{Z^n}\right) = - \int_\Psi D_{t,\psi} \dxi{\ff} \psi^n \mathrm{d}\psi = -\fav{D}_{t,Z^n} \dxi{\fav{Z^n}},\label{sm_eq:sgs_flux2}
\end{equation}
where $\fav{D}_{t,Z^n}$ refers to the eddy-diffusivity of the $\mathrm{n^{th}}$ moment. 
The consistency condition can be easily satisfied assuming that $D_{t,\psi}$ is independent of $\psi$, i.e, $D_{t,\psi}=\fav{D}_t$. Then Eq.~(\ref{sm_eq:sgs_flux2}) can be evaluated analytically, yielding
\begin{equation}
\left(\fav{u_i Z^n} - \fav{u}_i\fav{Z^n}\right) = -\int_\Psi  \fav{D}_{t} \dxi{\ff }\psi^n  \mathrm{d}\psi 
 				 				= -\fav{D}_{t}  \int_\Psi  \dxi{\ff \psi^n}  \mathrm{d}\psi 
								= -\fav{D}_{t} \dxi{\fav{Z^n}}	\label{sm_eq:sgs_flux3}
\end{equation}
Hence, the consistency condition recovers the Smagorinsky model for all moments. Furthermore, it follows that the eddy-diffusivities of all moments, $\fav{D}_{Z^n}$, are equal to $\fav{D}_{t}$.
\subsection{Consistent conditional flow parameters}
The consistent conditional flow parameters will be derived in this section. First, the consistency condition is derived. Afterwards, consistent formulations for each conditional flow parameter are presented. 
\subsubsection{Consistency condition}
The basis for the derivations of all parameters is the FDF transport equation (Eq.~(\ref{sm_eq:pdf_trans_chi})) employing the partial FDF derivatives from the presumed FDF approach (Eq.~(\ref{sm_eq:dFDFdtmodel}) and Eq.~(\ref{sm_eq:dFDFdximodel})) and the mixture fraction moment equations given by Eq.~(\ref{sm_eq:Z1trans}) and Eq.~(\ref{sm_eq:Z2trans}). Assuming that $D_{t,\psi}=\fav{D}_t$ and performing some algebraic transformations results in an equation that relates the conditional flow parameters to the mixture fraction moment evolutions, which read
\begin{equation}
\begin{split}
\frac{1}{2}\ddPsi{\orho\ff\cond{\chi_Z}} &+ \dPsi{}\left[\orho\ff\cond{\zeta_Z}(1-\psi)\right] 
-\ff\orho \cond{\zeta_Z}  = \\
&\orho \left(\fav{D} + \fav{D}_t\right) \left(\dxi{\fav{Z}}\dxi{\fav{Z}}\frac{\partial^2\ff}{\partial \fav{Z}^2} 
+2\dxi{\fav{Z}}\dxi{\fav{Z^2}}\frac{\partial^2\ff}{\partial\fav{Z}\partial \fav{Z^2}} 
+\dxi{\fav{Z^2}}\dxi{\fav{Z^2}}\frac{\partial^2\ff}{\partial \fav{Z^2}^2}\right) \\
&\left[\ol{\dot{S}}_\rho \left(1-\fav{Z}\right)\right]\frac{\partial\ff}{\partial{\fav{Z}}} +\left(\orho\fav{\chi}_Z - \ol{\dot{S}_\rho \left(2Z-Z^2\right)}  + \ol{\dot{S}}_\rho\fav{Z^2} \right)\frac{\partial\ff}{\partial{\fav{Z^2}}} 
-\ff\ol{\dot{S}}_\rho. \label{sm_eq:condFlowBasis2}
\end{split}
\end{equation}
\subsubsection{Conditional mixture fraction dissipation rate}
The conditional dissipation rate can be derived by considering that the instantaneous scalar dissipation rate of a scalar mixing field is defined and hence directly given by the local mixture fraction gradient and the mixture fraction diffusivity. It is, therefore, only indirectly affected by mass source terms. It is clear that the presence of mass source terms affects the scalar dissipation rate evolution by increasing or reducing scalar gradients over time. However, since we are interested in the instantaneous dissipation rate, we can neglect all mass source term effects in Eq.~(\ref{sm_eq:condFlowBasis2}) for deriving the conditional dissipation rate. Hence, we can obtain $\cond{\chi_Z}$ by integrating Eq.~(\ref{sm_eq:condFlowBasis2}) twice in mixture fraction sample space. The integration can be easily performed since
all variables, apart from $\ff$, are independent of $\psi$, and can therefore be factorized from the integral. Additionally, the order of integration and differentiation can be altered since the integration bounds are independent of the mixture fraction moments. Hence, the conditional mixture fraction dissipation can be obtained via
\begin{equation}
\ff\cond{\chi_Z} = 2  \left(\fav{D} + \fav{D}_t\right)
\left(
\dxi{\fav{Z}}\dxi{\fav{Z}}\frac{\partial^2\iif}{\partial \fav{Z}^2} 
+2\dxi{\fav{Z}}\dxi{\fav{Z^2}}\frac{\partial^2\iif}{\partial\fav{Z}\partial \fav{Z^2}} 
+\dxi{\fav{Z^2}}\dxi{\fav{Z^2}}\frac{\partial^2\iif}{\partial \fav{Z^2}^2} 
\right) +2\fav{\chi}_Z \frac{\partial\iif}{\partial{\fav{Z^2}}},
\label{sm_eq:condCHIexact}
\end{equation}
where a new function has been introduced for better readability, which is defined by
\begin{equation}
\iif  \left(\psi;\mathbf{x},t\right) = \iint_{\Zmin}^\psi \ff\left(\psi';\fav{Z},\fav{Z^2}\right)\mathrm{d}\psi'\mathrm{d}\psi', \label{sm_eq:iif_def} 
\end{equation}
For the modified beta distribution (Eq.~(\ref{sm_eq:scaledBeta})), an analytical solution can be derived for $\iif$ using integration by substitution
\begin{equation}
\begin{split}
\iif = 
&\frac{1}{B(a,b)\Delta Z} \iint_{\Zmin}^\psi {\psi^*}^{a-1} \left(1-\psi^*\right)^{b-1} \mathrm{d}\psi'\mathrm{d}\psi' 
=\frac{\Delta Z}{B(a,b)} \int_{0}^{\psi^*} B_{{\psi}^{*}}(a,b) \mathrm{d}{\psi'}^{*}  \\
=&\frac{\Delta Z}{B(a,b)}  \left[\psi^* B_{{\psi}^{*}}(a,b)  - B_{{\psi}^{*}}(a+1,b)\right], \label{sm_eq:iif_beta}
\end{split}
\end{equation}
where $B_{{\psi}^{*}}(a,b)$ is the incomplete beta function at ${\psi}^{*}$. $B_{{\psi}^{*}}(a,b)$ can be numerically evaluated using the method of continued fraction \citeapp{Cuyt2008}, which converges rapidly for sufficiently large variances. At the same time, the convergence rate is slow for tiny variances. Fortunately, the beta distribution can be well approximated by a delta distribution for those cases. Hence, it is computationally more favorable to switch to a delta distribution when the beta distribution is not sufficiently resolved by the sample space grid. For a delta distribution, an analytic solution exists for Eq.~(\ref{sm_eq:condCHIexact}) that reads
\begin{equation}
\ff\cond{\chi_Z} =  \ff2\left(\fav{D} + \fav{D}_t\right)\dxi{\fav{Z}}\dxi{\fav{Z}}.
\label{sm_eq:condCHIdelta}
\end{equation}
%In this study, a delta distribution is used when the variance falls below $5\cdot10^{-6}$. 
%%%%%%%% CONDITIONAL DIFFUSION RATE %%%%%%%%%
\subsubsection{Conditional mixture fraction diffusion rate}
The conditional diffusion rate can be determined from $\cond{\chi_Z}$ (Eq.~(\ref{sm_eq:condCHIexact})) and Eq.~(\ref{sm_eq:condDiffcondDiss2}) and reads
\begin{equation}
\begin{split}
\ff\cond{\xi_Z} =  & \fav{D}_t \left(\dxi{\fav{Z}}\dxi{\fav{Z}} 								\frac{\partial^2\fav{F}_Z }{\partial \fav{Z}^2} 
				+ 2  \dxi{\fav{Z}}\dxi{\fav{Z^2}} 							\frac{\partial^2\fav{F}_Z}{\partial \fav{Z}\fav{Z^2}}  
 				+  \dxi{\fav{Z^2}}\dxi{\fav{Z^2}}  							\frac{\partial^2\fav{F}_Z}{\partial \fav{Z^2}} \right)\\
				 &-\frac{1}{\orho}\dxi{} \left(\orho \fav{D} \dxi{\fav{Z}}\right) 							\frac{\partial\fav{F}_Z}{\partial \fav{Z}}  
                                   -\Biggl[\frac{1}{\orho}\dxi{} \left(\orho \fav{D}\dxi{\fav{Z^2}}\right) - \fav{\chi}_Z\Biggl]	\frac{\partial\fav{F}_Z}{\partial \fav{Z^2}^2}.\label{sm_eq:xiMdlwsrc}
\end{split} 
\end{equation}
Note that $\fav{F}_Z$ refers to the cumulative filtered density function (CDF), which is defined as $\fav{F}_Z=\int_{\Zmin}^\psi \ff\left(\psi';\fav{Z},\fav{Z^2}\right)\mathrm{d}\psi'$. For a modified beta distribution, $\fav{F}_Z$ is given by 
\begin{equation}
\begin{split}
 \fav{F}_Z = \frac{1}{B(a,b)\Delta Z} \int_{\Zmin}^\psi {\psi^*}^{a-1} \left(1-\psi^*\right)^{b-1} \mathrm{d}\psi'=\frac{B_{{\psi'}^{*}}(a,b)}{B(a,b)}.
\end{split}
\end{equation}
Similarly to $\ff\cond{\chi_Z}$, an analytical solution can be found for $\ff\cond{\xi_Z}$ if a delta distribution is employed, which reads
\begin{equation}
\begin{split}
\delta\left(\psi-\fav{Z}\right)\cond{\xi_Z} =  \delta\left(\psi-\fav{Z}\right)\frac{1}{\orho}\dxi{} \left(\orho \fav{D} \dxi{\fav{Z}}\right) 	.						\label{sm_eq:xiMdlDelta}
\end{split} 
\end{equation}
%%%%%%%% CONDITIONAL SOURCE TERM %%%%%%%%%
\subsubsection{Conditional normalized source term}
The conditional normalized mass source term can be obtained by inserting Eq.~(\ref{sm_eq:condCHIexact}) into Eq.~(\ref{sm_eq:condFlowBasis2}), which results in 
\begin{equation}
 (\psi-1)\dPsi{}\left(\orho\ff\cond{\zeta_Z}\right)  + 2 \ff \orho \cond{\zeta_Z} = 
 \ol{\dot{S}}_\rho \left(1-\fav{Z}\right) \frac{\partial\ff}{\partial \fav{Z}} + \left[ \ol{\dot{S}_\rho \left(2Z-Z^2\right)}  - \ol{\dot{S}}_\rho\fav{Z^2}\right]\frac{\partial\ff}{\partial \fav{Z^2}} + \ol{\dot{S}}_\rho\ff . \label{sm_eq:srcODE}
\end{equation}
For a given set of mixture fraction moments, Eq.~(\ref{sm_eq:srcODE}) resembles a first-order linear ordinary differential equation (ODE) that relates the conditional spray source term to the presumed FDF shape and mixture fraction moment source terms. An analytical solution can be found using the method of integrating factors that reads
\begin{equation}
\ff \cond{\zeta_Z} = 
  \frac{\ol{\dot{S}}_\rho \left(1-\fav{Z}\right) }{\orho\left(\psi-1\right)^2} 	   \frac{\partial \fav{F}_Z^*}{\partial \fav{Z}}      
+\frac{\ol{\dot{S}_\rho \left(2Z-Z^2\right)} -\ol{\dot{S}}_\rho\fav{Z^2} }{\orho\left(\psi-1\right)^2} \frac{\partial\fav{F}_Z^* }{\partial \fav{Z^2}} 
+\frac{\ol{\dot{S}}_\rho}{\orho\left(\psi-1\right)^2} 					                                          	         \fav{F}_Z^* , \label{sm_eq:condSrc} 
\end{equation}
where a new function $\fav{F}_Z^* = \int_{-\infty}^\psi(\psi'-1) \ff\mathrm{d} \psi' $ has been introduced. If a modified beta distribution is employed, $\fav{F}_Z^*$ is given by 
\begin{equation}
\fav{F}^*_Z 		=\frac{\Delta Z }{B\left(a,b\right)}\left[B_{\psi^*}\left(a+1,b\right) - \frac{1-\Zmin}{\Delta Z}B_{\psi^*}\left(a,b\right) \right] \label{sm_eq:CDFstar},
\end{equation}
while Eq.~(\ref{sm_eq:condSrc}) reduces to 
\begin{equation}
\delta\left(\psi-\fav{Z}\right)\cond{\zeta_Z} = \delta\left(\psi-\fav{Z}\right)\frac{\ol{\dot{S}}_\rho}{\orho},  \label{sm_eq:condSrcDelta} 
\end{equation}
when a delta distribution is used.


==> figures/epsilon.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4534.00,4194.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(434,2840){\makebox(0,0)[r]{\strut{}-5}}%
      \put(434,3237){\makebox(0,0)[r]{\strut{} 0}}%
      \put(434,3633){\makebox(0,0)[r]{\strut{} 5}}%
      \put(566,2541){\makebox(0,0){\strut{}}}%
      \put(963,2541){\makebox(0,0){\strut{}}}%
      \put(1359,2541){\makebox(0,0){\strut{}}}%
      \put(1756,2541){\makebox(0,0){\strut{}}}%
      \put(2153,2541){\makebox(0,0){\strut{}}}%
      \put(2549,2541){\makebox(0,0){\strut{}}}%
      \put(2946,2541){\makebox(0,0){\strut{}}}%
      \put(3342,2541){\makebox(0,0){\strut{}}}%
      \put(3739,2541){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(82,3236){\rotatebox{-270}{\makebox(0,0){\strut{}$y$~[mm]}}}%
      \put(1242,3538){\makebox(0,0){\strut{}\textcolor{white}{$\avg{\orho\fav{D}_t}$~[kg/(m$\cdot$s)]}}}%
      \csname LTb\endcsname%%
      \put(4108,2760){\makebox(0,0)[l]{\strut{}$10^{-4}$}}%
      \put(4108,3078){\makebox(0,0)[l]{\strut{}$10^{-3}$}}%
      \put(4108,3395){\makebox(0,0)[l]{\strut{}$10^{-2}$}}%
      \put(4108,3712){\makebox(0,0)[l]{\strut{}$10^{-1}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(434,1721){\makebox(0,0)[r]{\strut{}-5}}%
      \put(434,2118){\makebox(0,0)[r]{\strut{} 0}}%
      \put(434,2514){\makebox(0,0)[r]{\strut{} 5}}%
      \put(566,1422){\makebox(0,0){\strut{}}}%
      \put(963,1422){\makebox(0,0){\strut{}}}%
      \put(1359,1422){\makebox(0,0){\strut{}}}%
      \put(1756,1422){\makebox(0,0){\strut{}}}%
      \put(2153,1422){\makebox(0,0){\strut{}}}%
      \put(2549,1422){\makebox(0,0){\strut{}}}%
      \put(2946,1422){\makebox(0,0){\strut{}}}%
      \put(3342,1422){\makebox(0,0){\strut{}}}%
      \put(3739,1422){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(82,2117){\rotatebox{-270}{\makebox(0,0){\strut{}$y$~[mm]}}}%
      \put(991,2419){\makebox(0,0){\strut{}\textcolor{white}{$\avg{\fav{\chi}_Z}$~[1/s]}}}%
      \csname LTb\endcsname%%
      \put(4108,1642){\makebox(0,0)[l]{\strut{}$10^{0}$}}%
      \put(4108,1959){\makebox(0,0)[l]{\strut{}$10^{1}$}}%
      \put(4108,2276){\makebox(0,0)[l]{\strut{}$10^{2}$}}%
      \put(4108,2593){\makebox(0,0)[l]{\strut{}$10^{3}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(434,603){\makebox(0,0)[r]{\strut{}-5}}%
      \put(434,1000){\makebox(0,0)[r]{\strut{} 0}}%
      \put(434,1396){\makebox(0,0)[r]{\strut{} 5}}%
      \put(566,304){\makebox(0,0){\strut{} 0}}%
      \put(963,304){\makebox(0,0){\strut{} 5}}%
      \put(1359,304){\makebox(0,0){\strut{}10}}%
      \put(1756,304){\makebox(0,0){\strut{}15}}%
      \put(2153,304){\makebox(0,0){\strut{}20}}%
      \put(2549,304){\makebox(0,0){\strut{}25}}%
      \put(2946,304){\makebox(0,0){\strut{}30}}%
      \put(3342,304){\makebox(0,0){\strut{}35}}%
      \put(3739,304){\makebox(0,0){\strut{}40}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(82,999){\rotatebox{-270}{\makebox(0,0){\strut{}$y$~[mm]}}}%
      \put(2152,84){\makebox(0,0){\strut{}$x$~[mm]}}%
      \put(872,1301){\makebox(0,0){\strut{}\textcolor{white}{$\avg{\fav{\epsilon}}$~[-]}}}%
      \csname LTb\endcsname%%
      \put(4108,524){\makebox(0,0)[l]{\strut{}1}}%
      \put(4108,999){\makebox(0,0)[l]{\strut{}2}}%
      \put(4108,1475){\makebox(0,0)[l]{\strut{}3}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{epsilon}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/verification_results.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3628.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(288,720){\makebox(0,0)[r]{\strut{}$-1800$}}%
      \csname LTb\endcsname%%
      \put(288,1135){\makebox(0,0)[r]{\strut{}$-1200$}}%
      \csname LTb\endcsname%%
      \put(288,1550){\makebox(0,0)[r]{\strut{}$-600$}}%
      \csname LTb\endcsname%%
      \put(288,1965){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(432,480){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(985,480){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%%
      \put(1537,480){\makebox(0,0){\strut{}$0.2$}}%
      \csname LTb\endcsname%%
      \put(2090,480){\makebox(0,0){\strut{}$0.3$}}%
      \csname LTb\endcsname%%
      \put(2642,480){\makebox(0,0){\strut{}$0.4$}}%
      \csname LTb\endcsname%%
      \put(3195,480){\makebox(0,0){\strut{}$0.5$}}%
      \put(3339,720){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3339,1135){\makebox(0,0)[l]{\strut{}$600$}}%
      \put(3339,1550){\makebox(0,0)[l]{\strut{}$1200$}}%
      \put(3339,1965){\makebox(0,0)[l]{\strut{}$1800$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-312,1446){\rotatebox{-270}{\makebox(0,0){\strut{}$\cond{\chi_Z}, \cond{\xi_Z}$~[1/s]}}}%
      \put(3915,1446){\rotatebox{-270}{\makebox(0,0){\strut{}$\cond{\zeta_Z}$~[1/s]}}}%
      \put(1813,240){\makebox(0,0){\strut{}$\psi$~[-]}}%
      \csname LTb\endcsname%%
      \put(354,2685){\makebox(0,0)[l]{\strut{}LCFP~~~}}%
      \csname LTb\endcsname%%
      \put(354,2445){\makebox(0,0)[l]{\strut{}$\cond{\chi_Z}$~~~}}%
      \csname LTb\endcsname%%
      \put(1540,2685){\makebox(0,0)[l]{\strut{}WENO5U}}%
      \csname LTb\endcsname%%
      \put(1540,2445){\makebox(0,0)[l]{\strut{}$\cond{\xi_Z}$~~~}}%
      \csname LTb\endcsname%%
      \put(2726,2685){\makebox(0,0)[l]{\strut{}WENO5~~}}%
      \csname LTb\endcsname%%
      \put(2726,2445){\makebox(0,0)[l]{\strut{}$\cond{\zeta_Z}$~~~}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{verification_results}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/verify.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3628.00,3174.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(230,2171){\makebox(0,0)[r]{\strut{}-5}}%
      \put(230,2500){\makebox(0,0)[r]{\strut{} 0}}%
      \put(230,2828){\makebox(0,0)[r]{\strut{} 5}}%
      \put(362,1885){\makebox(0,0){\strut{}}}%
      \put(691,1885){\makebox(0,0){\strut{}}}%
      \put(1020,1885){\makebox(0,0){\strut{}}}%
      \put(1348,1885){\makebox(0,0){\strut{}}}%
      \put(1677,1885){\makebox(0,0){\strut{}}}%
      \put(2006,1885){\makebox(0,0){\strut{}}}%
      \put(2335,1885){\makebox(0,0){\strut{}}}%
      \put(2663,1885){\makebox(0,0){\strut{}}}%
      \put(2992,1885){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-122,2499){\rotatebox{-270}{\makebox(0,0){\strut{}$y$~[mm]}}}%
      \put(1268,2720){\makebox(0,0){\strut{}Droplet Diameter~[m]}}%
      \csname LTb\endcsname%%
      \put(3321,2380){\makebox(0,0)[l]{\strut{}$10^{-6}$}}%
      \put(3321,2775){\makebox(0,0)[l]{\strut{}$10^{-5}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(230,1245){\makebox(0,0)[r]{\strut{}-5}}%
      \put(230,1574){\makebox(0,0)[r]{\strut{} 0}}%
      \put(230,1902){\makebox(0,0)[r]{\strut{} 5}}%
      \put(362,959){\makebox(0,0){\strut{}}}%
      \put(691,959){\makebox(0,0){\strut{}}}%
      \put(1020,959){\makebox(0,0){\strut{}}}%
      \put(1348,959){\makebox(0,0){\strut{}}}%
      \put(1677,959){\makebox(0,0){\strut{}}}%
      \put(2006,959){\makebox(0,0){\strut{}}}%
      \put(2335,959){\makebox(0,0){\strut{}}}%
      \put(2663,959){\makebox(0,0){\strut{}}}%
      \put(2992,959){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-122,1573){\rotatebox{-270}{\makebox(0,0){\strut{}$y$~[mm]}}}%
      \put(621,1794){\makebox(0,0){\strut{}\color{white}{$\fav{Z}$ [-]}}}%
      \csname LTb\endcsname%%
      \put(3321,1179){\makebox(0,0)[l]{\strut{}0.00}}%
      \put(3321,1442){\makebox(0,0)[l]{\strut{}0.10}}%
      \put(3321,1705){\makebox(0,0)[l]{\strut{}0.20}}%
      \put(3321,1968){\makebox(0,0)[l]{\strut{}0.30}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(230,319){\makebox(0,0)[r]{\strut{}-5}}%
      \put(230,648){\makebox(0,0)[r]{\strut{} 0}}%
      \put(230,976){\makebox(0,0)[r]{\strut{} 5}}%
      \put(362,33){\makebox(0,0){\strut{} 0}}%
      \put(691,33){\makebox(0,0){\strut{} 5}}%
      \put(1020,33){\makebox(0,0){\strut{}10}}%
      \put(1348,33){\makebox(0,0){\strut{}15}}%
      \put(1677,33){\makebox(0,0){\strut{}20}}%
      \put(2006,33){\makebox(0,0){\strut{}25}}%
      \put(2335,33){\makebox(0,0){\strut{}30}}%
      \put(2663,33){\makebox(0,0){\strut{}35}}%
      \put(2992,33){\makebox(0,0){\strut{}40}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(-122,647){\rotatebox{-270}{\makebox(0,0){\strut{}$y$~[mm]}}}%
      \put(1677,-143){\makebox(0,0){\strut{}$x$~[mm]}}%
      \put(714,868){\makebox(0,0){\strut{}\color{white}{$\Zvar$ [-]}}}%
      \csname LTb\endcsname%%
      \put(3321,253){\makebox(0,0)[l]{\strut{}0.000}}%
      \put(3321,516){\makebox(0,0)[l]{\strut{}0.010}}%
      \put(3321,779){\makebox(0,0)[l]{\strut{}0.020}}%
      \put(3321,1042){\makebox(0,0)[l]{\strut{}0.030}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{verify}}%
    \gplfronttext
  \end{picture}%
\endgroup

